Efficient Column-Wise N:M Pruning on RISC-V CPU

In deep learning frameworks, weight pruning is a widely used technique for improving computational efficiency by reducing the size of large models. This is especially critical for convolutional operators, which often act as performance bottlenecks in convolutional neural networks (CNNs). However, the effectiveness of pruning heavily depends on how it is implemented, as different methods can significantly impact both computational performance and memory footprint. In this work, we propose a column-wise N:M pruning strategy applied at the tile level and modify XNNPACK to enable efficient execution of pruned models on the RISC-V vector architecture. Additionally, we propose fusing the operations of im2col and data packing to minimize redundant memory accesses and memory overhead. To further optimize performance, we incorporate AITemplate's profiling technique to identify the optimal implementation for each convolutional operator. Our proposed approach effectively increases ResNet inference throughput by as much as 4.0x, and preserves ImageNet top-1 accuracy within 2.1\% of the dense baseline.

==> experiment_pruned_models.tex <==
\subsection{Performance of Different Pruned Models}

As detailed in Sections~\ref{subsec:method_Microkernel_Design} and \ref{subsec:expr_setup}, we perform column-wise N:M pruning on ResNet (18, 34, 50, 101, 152), MobileNet-V2, and DenseNet-121 for end-to-end benchmarking. Each network retains the NHWC data layout until the first major stage, after which we perform a single conversion to CNHW: after \textbf{Layer 1} in ResNet, after \textbf{Block 1} in MobileNet‑V2, and after \textbf{DenseBlock 2} in DenseNet‑121.
Pruning is applied immediately after this layout transformation. Because the vast majority of parameters in ResNet and MobileNet-V2 lie beyond Layer 1/Block 1, the global sparsity closely matches $100 \times \text{sparsity\_ratio}\,\%$. By contrast, the later conversion point in DenseNet-121 exposes roughly half of the weights to pruning, yielding an overall sparsity of about $50 \times \text{sparsity\_ratio}\,\%$.

Table ~\ref{tab:model_accuracy_runtime_7subtables} presents runtime and top-1 accuracy for various sparsity\_ratio. For ResNet models with depths less than 50, combining the mixed NHWC/CNHW data layout, pruning, and distinct LMUL configurations per operator achieves up to a 4.0$\times$ speedup over the NHWC baseline, with less than 2.1\% accuracy loss, and up to 0.3\% accuracy gain at a sparsity\_ratio of 0.25. For ResNet models with depths of 50 or greater, the speedups are up to 3.2$\times$ over the NHWC baseline, and up to 1.9$\times$ compared to dense implementations using the mixed NHWC/CNHW layout, again with less than 1.9\% accuracy loss.

For MobileNet-V2, the microkernel achieves a speed-up of up to $1.4\times$ relative to the dense NHWC baseline.  Nevertheless, imposing the proposed pruning pattern on this depth-wise–separable network leads to a substantial Top-1 accuracy drop—as high as 12 percentage points—suggesting that MobileNet-V2 is more sensitive to structured sparsity than the other models considered.

For DenseNet-121, the mixed NHWC/CNHW memory layout limits the hardware gains, yielding a maximum throughput improvement of roughly $8\%$ over the NHWC baseline. In contrast to MobileNet-V2, DenseNet-121 tolerates pruning well: at a sparsity\_ratio of 0.5 the Top-1 accuracy increases by 0.6 percentage points, and at a ratio of 0.75 the loss is confined to only 0.9 percentage points.  Thus, our column-wise N:M pruning delivers an attractive accuracy–sparsity trade-off for DenseNet-121 while still providing modest performance gains.

These results indicate our method is more effective for middle-weight to heavyweight models, such as ResNet, rather than lightweight models like MobileNet and DenseNet. Regarding accuracy, our pruning method yields improved or only minor accuracy loss in models dominated by spatial convolution operators, while lightweight models relying primarily on point-wise and depthwise convolutions may experience severe accuracy losses.
% \input{figure_expr/Model_expr.tikz}
\input{figure_expr/Model_expr_new_table.tikz}
